Explicit Hochschild Cocycles for Gentle Algebras

Hochschild cohomology is crucial for understanding deformation theory. In arXiv:2304.10223, we have computed the Hochschild cohomology for gentle algebras of punctured surfaces. The construction of that paper is rather implicit and fails if the punctured surface has only a single puncture. In the present note, we supplement the earlier method by providing an explicit construction of Hochschild cocycles which also succeeds in the case of a single puncture.

==> even/cup_bracket.tex <==
\subsection{Cup product and Gerstenhaber bracket}
In this section, we determine cup product and Gerstenhaber bracket on Hochschild cohomology of $ \Gtl \cA $. More precisely, we have already determined both in \paperone\ under the assumption [NL2]. In the present section, we extend the statement of \paperone\ to the case without [NL2]. In fact, the only change is the knowledge that the ordinary even classes exist.

